Model category structures \`a la Thomason on 2-Cat

In his paper "Th\'eories homotopiques des 2-cat\'egories", Jonathan Chiche studies homotopy theories on 2-Cat, the category of small strict 2-categories, given by classes of weak equivalences which he calls basic localizers of 2-Cat. These basic localizers of 2-Cat are a 2-categorical generalization of the notion of a basic localizer introduced by Grothendieck in "Pursuing stacks". In this paper, we deduce from the results of Jonathan Chiche and results we have obtained with Georges Maltsiniotis that for essentially every basic localizer W of 2-Cat, there exists a model category structure \`a la Thomason on 2-Cat whose weak equivalences are given by W. We show that these model category structures model exactly combinatorial left Bousfield localization of the classical homotopy theory of simplicial sets.

==> smfref.tex <==
\makeatletter

% vielle version de l'environnement thebibliography de smfart.cls (la nouvelle
% n'est pas compatible avec hyperref)
\renewenvironment{thebibliography}[1]{%
  \bibliosection*{\refname}%
  \normalfont\labelsep .5em\relax
  \renewcommand\theenumiv{\arabic{enumiv}}\let\p@enumiv\@empty
  \list{\@biblabel{\theenumiv}}{\settowidth\labelwidth{\@biblabel{#1}}%
    \itemindent 0pt
    \leftmargin\labelwidth \advance\leftmargin\labelsep
    \usecounter{enumiv}}%
    \itemsep 0.1\baselineskip plus0.1\baselineskip
        minus0.1\baselineskip
    \bibliofont
  \sloppy \clubpenalty\@M \widowpenalty\clubpenalty
  \sfcode`\.=\@m
}{%
  \def\@noitemerr{\@latex@warning{Empty `thebibliography' environment}}%
  \endlist
}

% les liens internes vers les théorèmes ne marchent pas out-of-the-box avec
% smfart.cls
\def\@begintheorem#1#2[#3]{%
  \def\@theoremhead{\normalfont\the\thm@headfont
    \@ifempty{#1}{\let\thmname\@gobble}{\let\thmname\@iden}%
    \@ifempty{#2}{\let\thmnumber\@gobble}{\let\thmnumber\@iden}%
    \@ifempty{#3}{\let\thmnote\@gobble}{\let\thmnote\@iden}%
    \thm@swap\swappedhead\thmhead{#1}{#2}{#3}}%
  \sbox\@tempboxa{\@theoremhead}%
  \ifdim\wd\@tempboxa>0.7\linewidth \smf@skippttrue\fi
  \ifsmf@skippt
    \global\smf@skipptfalse
    \item [\thm@indent]%
          {\sloppy\@theoremhead\parskip\z@\@@par}%
    \nobreak\everypar{}%
    \let\thmheadnl\relax
  \else
    \item[\hskip\labelsep\thm@indent\unhbox\@tempboxa\the\thm@headpunct]%
%%    \hskip\z@\ignorespaces
  \fi
  \@restorelabelsep
  \thmheadnl % possibly a newline.
  \hypertarget{\csname @currentHref\endcsname}{}
  \ignorespaces}

\makeatother

